DBNode: A Decentralized Storage System for Big Data Storage in Consortium Blockchains

Storing big data directly on a blockchain poses a substantial burden due to the need to maintain a consistent ledger across all nodes. Numerous studies in decentralized storage systems have been conducted to tackle this particular challenge. Most state-of-the-art research concentrates on developing a general storage system that can accommodate diverse blockchain categories. However, it is essential to recognize the unique attributes of a consortium blockchain, such as data privacy and access control. Beyond ensuring high performance, these specific needs are often overlooked by general storage systems. This paper proposes a decentralized storage system for Hyperledger Fabric, which is a well-known consortium blockchain. First, we employ erasure coding to partition files, subsequently organizing these chunks into a hierarchical structure that fosters efficient and dependable data storage. Second, we design a two-layer hash-slots mechanism and a mirror strategy, enabling high data availability. Third, we design an access control mechanism based on a smart contract to regulate file access.

==> figures/spec_data1.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}[scale=.9]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
axis line style={white!80!black},
legend cell align={left},
legend style={fill opacity=0.2, draw opacity=1, text opacity=.8, draw=none, at={(0,1)},anchor=north west},
tick align=outside,
tick pos=left,
x grid style={white!80!black},
xlabel=\textcolor{white!15!black}{Wavelength (nm)},
xmajorgrids,
xmin=441.05, xmax=659.95,
xtick style={color=white!15!black},
y grid style={white!80!black},
ylabel=\textcolor{white!15!black}{Scaled photon count},
ymajorgrids,
ymin=-0.0308958739042282, ymax=0.648813351988792,
ytick style={color=white!15!black}
]
\addplot [semithick, color0]
table {%
650 0.00721221417188644
649 0.000139188021421432
648 0.0139264650642872
647 0.00380880385637283
646 0.018744895234704
645 0.00236091949045658
644 0.0121939703822136
643 0
642 0.0140484310686588
641 0.00704936310648918
640 0.050310380756855
639 0.0895640999078751
638 0.0919252187013626
637 0.130353525280952
636 0.16830974817276
635 0.192479372024536
634 0.211737751960754
633 0.228472948074341
632 0.254152148962021
631 0.272481709718704
630 0.263224959373474
629 0.283178180456161
628 0.300138682126999
627 0.318926692008972
626 0.332062393426895
625 0.344147056341171
624 0.369364023208618
623 0.38850536942482
622 0.391135036945343
621 0.416680991649628
620 0.425578027963638
619 0.441174387931824
618 0.456629365682602
617 0.480232805013657
616 0.490295976400375
615 0.505992412567139
614 0.528041660785675
613 0.562791883945465
612 0.553070306777954
611 0.551680684089661
610 0.562111377716064
609 0.569194555282593
608 0.557927370071411
607 0.556699693202972
606 0.535601139068604
605 0.542814671993256
604 0.512723743915558
603 0.4959796667099
602 0.499781876802444
601 0.471120804548264
600 0.437465041875839
599 0.445093035697937
598 0.422111302614212
597 0.421041488647461
596 0.409243494272232
595 0.400996148586273
594 0.397817850112915
593 0.392813056707382
592 0.381760358810425
591 0.36505925655365
590 0.34325635433197
589 0.347455650568008
588 0.326181918382645
587 0.316925436258316
586 0.325245767831802
585 0.31362396478653
584 0.298105180263519
583 0.305068343877792
582 0.269747585058212
581 0.267800897359848
580 0.243315666913986
579 0.226844936609268
578 0.241527944803238
577 0.223931223154068
576 0.215093046426773
575 0.231847763061523
574 0.191984891891479
573 0.198843210935593
572 0.171780407428741
571 0.162781119346619
570 0.16948726773262
569 0.149642556905746
568 0.142378360033035
567 0.141989931464195
566 0.120236307382584
565 0.131258904933929
564 0.110362224280834
563 0.0993513092398643
562 0.100167155265808
561 0.0902073532342911
560 0.0996171683073044
559 0.103642202913761
558 0.0682813227176666
557 0.0924751609563828
556 0.0782703682780266
555 0.0644536241889
554 0.0884837806224823
553 0.0892375260591507
552 0.0672072619199753
551 0.0647661909461021
550 0.0442351475358009
549 0.0543608032166958
548 0.0604598335921764
547 0.0380808189511299
546 0.0607272982597351
545 0.0490878969430923
544 0.0424884036183357
543 0.0590154677629471
542 0.0484637171030045
541 0.0688058137893677
540 0.042164258658886
539 0.0259125605225563
538 0.061937503516674
537 0.0290007926523685
536 0.0308153871446848
535 0.0606654211878777
534 0.0287332870066166
533 0.0423526279628277
532 0.0388693101704121
531 0.0216359440237284
530 0.0557848289608955
529 0.035499706864357
528 0.0348295122385025
527 0.0484343431890011
526 0.0436210185289383
525 0.0571794584393501
524 0.0788047611713409
523 0.0630588084459305
522 0.0729930102825165
521 0.0910252928733826
520 0.109725780785084
519 0.117094673216343
518 0.0984890833497047
517 0.117230027914047
516 0.105099447071552
515 0.0887063294649124
514 0.103146359324455
513 0.0874311029911041
512 0.0707721561193466
511 0.0777622759342194
510 0.0525237321853638
509 0.0709585249423981
508 0.0445900410413742
507 0.0321151465177536
506 0.06642846763134
505 0.0460884124040604
504 0.0395625755190849
503 0.0550230741500854
502 0.028115214779973
501 0.0528375804424286
500 0.0395957455039024
499 0.0262600239366293
498 0.0416697673499584
497 0.033947579562664
496 0.0253244023770094
495 0.045010719448328
494 0.00920469686388969
493 0.0270718950778246
492 0.0190813969820738
491 0.00744638405740261
490 0.0291463527828455
489 0.0194873567670584
488 0.0123096965253353
487 0.0311589688062668
486 0.00115368887782097
485 0.016579357907176
484 0.0196601562201977
483 0.000694006681442261
482 0.0224154777824879
481 0.0162200033664703
480 0.0204709842801094
479 0.0315813459455967
478 0
477 0.0229706019163132
476 0.0272943396121264
475 0.0148077569901943
474 0.0346031673252583
473 0.0208246894180775
472 0.0128462985157967
471 0.0344281531870365
470 0.0110536236315966
469 0.0357199609279633
468 0.0192581452429295
467 0
466 0.0311304721981287
465 0.0126256607472897
464 0.00686400942504406
463 0.0337513759732246
462 0.00234591029584408
461 0.0267645996063948
460 0.0175804607570171
459 0
458 0.0218623615801334
457 0.0113786607980728
456 0.0137818865478039
455 0.0254226438701153
454 0.0247365385293961
453 0.0244207791984081
452 0.0293088722974062
451 0.00634961575269699
};
\addlegendentry{Pure}
\addplot [semithick, color1]
table {%
650 0
649 0
648 0
647 0
646 0
645 0
644 0
643 0
642 0
641 0
640 0.0308854281902313
639 0.0836381018161774
638 0.0891208201646805
637 0.14664551615715
636 0.19401541352272
635 0.231337457895279
634 0.254254996776581
633 0.286266088485718
632 0.321298897266388
631 0.347829163074493
630 0.32298544049263
629 0.348391383886337
628 0.376852482557297
627 0.385548621416092
626 0.402199238538742
625 0.411120235919952
624 0.443412810564041
623 0.46679499745369
622 0.452298432588577
621 0.484301179647446
620 0.47666397690773
619 0.480782747268677
618 0.489961862564087
617 0.509634733200073
616 0.511308968067169
615 0.528131365776062
614 0.523296713829041
613 0.568536937236786
612 0.554349184036255
611 0.556738913059235
610 0.566708207130432
609 0.58233916759491
608 0.573827624320984
607 0.583814799785614
606 0.563462018966675
605 0.586624026298523
604 0.563400328159332
603 0.558120131492615
602 0.586721122264862
601 0.565113723278046
600 0.533593952655792
599 0.570681095123291
598 0.541920006275177
597 0.558816730976105
596 0.552180469036102
595 0.571923851966858
594 0.581033706665039
593 0.577118217945099
592 0.587414562702179
591 0.576954066753387
590 0.557276010513306
589 0.567119121551514
588 0.55100554227829
587 0.54552686214447
586 0.568659663200378
585 0.560016989707947
584 0.544931173324585
583 0.549527645111084
582 0.499767035245895
581 0.49566051363945
580 0.442649930715561
579 0.430459350347519
578 0.439331978559494
577 0.410786628723145
576 0.397578209638596
575 0.419575154781342
574 0.356054544448853
573 0.365533173084259
572 0.318728536367416
571 0.30748838186264
570 0.307666718959808
569 0.274179011583328
568 0.269453018903732
567 0.270268231630325
566 0.220246821641922
565 0.235452890396118
564 0.20659813284874
563 0.180060982704163
562 0.182383477687836
561 0.166915029287338
560 0.17619377374649
559 0.17844346165657
558 0.117941595613956
557 0.150715708732605
556 0.135855600237846
555 0.106011472642422
554 0.153741091489792
553 0.149211496114731
552 0.11544393748045
551 0.0966128557920456
550 0.0663978978991508
549 0.0828118026256561
548 0.0940896198153496
547 0.0476076938211918
546 0.0845174193382263
545 0.060472346842289
544 0.0474771149456501
543 0.078641876578331
542 0.0590433515608311
541 0.0956838876008987
540 0.0497029460966587
539 0.0264275595545769
538 0.0762968361377716
537 0.0163723975419998
536 0.0249284412711859
535 0.0655405521392822
534 0.00476130098104477
533 0.0250784009695053
532 0.0324701406061649
531 0
530 0.0483458787202835
529 0.0101159811019897
528 0.0087602399289608
527 0.0227706842124462
526 0.0170124676078558
525 0.0302450750023127
524 0.0634454861283302
523 0.0304743349552155
522 0.0389440730214119
521 0.0657359510660172
520 0.0941575020551682
519 0.114433594048023
518 0.0777212381362915
517 0.112271472811699
516 0.0955325216054916
515 0.0723888874053955
514 0.0997070968151093
513 0.0827361717820168
512 0.0614995360374451
511 0.0729124993085861
510 0.0399557538330555
509 0.0653509497642517
508 0.0270220972597599
507 0.00808505155146122
506 0.063316248357296
505 0.0356131047010422
504 0.0282945334911346
503 0.0441509000957012
502 0.0113403182476759
501 0.0452808775007725
500 0.0315222702920437
499 0.00838768482208252
498 0.030874315649271
497 0.0204923152923584
496 0.00341213867068291
495 0.0402427911758423
494 0
493 0.00857250206172466
492 0
491 0
490 0.0113102737814188
489 0
488 0
487 0.00716127082705498
486 0
485 0
484 0
483 0
482 0
481 0
480 0
479 0.00747537426650524
478 0
477 0
476 0.0124205928295851
475 0
474 0.0142969973385334
473 0.00233200192451477
472 0
471 0.0226709619164467
470 0
469 0.0239057317376137
468 0.00459364615380764
467 0
466 0.0198479015380144
465 0
464 0
463 0.0232024230062962
462 0
461 0.0130661502480507
460 0.0100967213511467
459 0
458 0.0137269087135792
457 4.47109341621399e-05
456 0.00307325087487698
455 0.0159360021352768
454 0.0114260818809271
453 0.015860928222537
452 0.0252320561558008
451 0
};
\addlegendentry{Minor Adulteration}

\addplot [semithick, color3]
table {%
650 0.0272618718445301
649 0.0253714136779308
648 0.0363947376608849
647 0.0327915549278259
646 0.0455745235085487
645 0.0456829592585564
644 0.053199328482151
643 0.0509699024260044
642 0.0600532218813896
641 0.0658651888370514
640 0.0949893221259117
639 0.145586222410202
638 0.158568263053894
637 0.187256693840027
636 0.224427491426468
635 0.24943283200264
634 0.271087884902954
633 0.282613515853882
632 0.300876021385193
631 0.306917011737823
630 0.295168370008469
629 0.309031069278717
628 0.316425889730453
627 0.323767244815826
626 0.329145222902298
625 0.331506133079529
624 0.346958875656128
623 0.359735161066055
622 0.352263301610947
621 0.368393540382385
620 0.36542621254921
619 0.370462715625763
618 0.376654744148254
617 0.390974849462509
616 0.392947018146515
615 0.399568974971771
614 0.409270733594894
613 0.437150448560715
612 0.428752094507217
611 0.433305650949478
610 0.43461549282074
609 0.44710436463356
608 0.442440867424011
607 0.451467245817184
606 0.441410571336746
605 0.459003984928131
604 0.444171220064163
603 0.451382994651794
602 0.475514948368073
601 0.469439446926117
600 0.454490005970001
599 0.490029096603394
598 0.480147063732147
597 0.499478548765182
596 0.504570007324219
595 0.516847193241119
594 0.526774644851685
593 0.536091506481171
592 0.544784307479858
591 0.536472856998444
590 0.522703468799591
589 0.532679975032806
588 0.51915043592453
587 0.519951522350311
586 0.536789238452911
585 0.533825933933258
584 0.522284269332886
583 0.525058627128601
582 0.4905806183815
581 0.486448645591736
580 0.448917746543884
579 0.438024789094925
578 0.44244509935379
577 0.424644738435745
576 0.406964153051376
575 0.417811840772629
574 0.376350343227386
573 0.378158420324326
572 0.349924385547638
571 0.342304408550262
570 0.340285629034042
569 0.318775504827499
568 0.310271203517914
567 0.307357788085938
566 0.275163471698761
565 0.284355908632278
564 0.265328377485275
563 0.243917644023895
562 0.240756839513779
561 0.234771847724915
560 0.233885765075684
559 0.228495478630066
558 0.196276783943176
557 0.215973138809204
556 0.202758848667145
555 0.177276045084
554 0.201141268014908
553 0.19718411564827
552 0.169965147972107
551 0.148539990186691
550 0.129832550883293
549 0.129818737506866
548 0.132893115282059
547 0.0991212576627731
546 0.110127225518227
545 0.0978996008634567
544 0.0793637111783028
543 0.094158411026001
542 0.0822743624448776
541 0.101758651435375
540 0.065587118268013
539 0.0524450913071632
538 0.0847541615366936
537 0.0480769574642181
536 0.0474207997322083
535 0.0737585723400116
534 0.0425509810447693
533 0.0521877519786358
532 0.05025689676404
531 0.036045141518116
530 0.0643533319234848
529 0.0524260103702545
528 0.0517534017562866
527 0.0667091310024261
526 0.0626166835427284
525 0.0761216953396797
524 0.104548238217831
523 0.0913234204053879
522 0.100511111319065
521 0.119241796433926
520 0.137465998530388
519 0.141630291938782
518 0.134446620941162
517 0.147693499922752
516 0.135537594556808
515 0.121267482638359
514 0.133386209607124
513 0.11674776673317
512 0.102420695126057
511 0.103936783969402
510 0.0816780105233192
509 0.0977392345666885
508 0.067410483956337
507 0.0548072382807732
506 0.083329439163208
505 0.0701462253928185
504 0.0570349432528019
503 0.0650994032621384
502 0.046098355203867
501 0.0659113824367523
500 0.0536341220140457
499 0.0436857976019382
498 0.0504669174551964
497 0.0501091443002224
496 0.0425415113568306
495 0.0593661814928055
494 0.0289258752018213
493 0.0415303893387318
492 0.0350132547318935
491 0.026697862893343
490 0.0409173518419266
489 0.0348619297146797
488 0.0328382849693298
487 0.0486729666590691
486 0.0211677365005016
485 0.0375280901789665
484 0.0356453061103821
483 0.022081907838583
482 0.0371522381901741
481 0.0300892665982246
480 0.0326631031930447
479 0.0416446179151535
478 0.0134122353047132
477 0.0376300066709518
476 0.0356119126081467
475 0.0254053063690662
474 0.043928999453783
473 0.0314866825938225
472 0.0200276337563992
471 0.0411010682582855
470 0.0145447254180908
469 0.0388107039034367
468 0.0242502931505442
467 0.00700809434056282
466 0.0340696722269058
465 0.0175979547202587
464 0.00847022049129009
463 0.0344336628913879
462 0.00539827346801758
461 0.0290270857512951
460 0.0180901736021042
459 0.00176279991865158
458 0.0224289149045944
457 0.0103520527482033
456 0.0118928253650665
455 0.027155352756381
454 0.0251910090446472
453 0.0192321799695492
452 0.0250522941350937
451 0.00342648476362228
};
\addlegendentry{Major Adulteration}
\addplot [semithick, color2]
table {%
650 0
649 0
648 0.00457106158137321
647 0
646 0.0101089179515839
645 0
644 0
643 0
642 0.0115335658192635
641 0.00304093956947327
640 0.0572072491049767
639 0.0872213467955589
638 0.0884950906038284
637 0.115935452282429
636 0.154910862445831
635 0.166037142276764
634 0.195611596107483
633 0.203844368457794
632 0.210380464792252
631 0.219168812036514
630 0.178465962409973
629 0.195523530244827
628 0.196194857358932
627 0.178822368383408
626 0.189390033483505
625 0.181044965982437
624 0.197884917259216
623 0.221930205821991
622 0.186549246311188
621 0.210339277982712
620 0.200703859329224
619 0.199540197849274
618 0.222125709056854
617 0.221779406070709
616 0.230606913566589
615 0.234613120555878
614 0.225758105516434
613 0.253526359796524
612 0.246158212423325
611 0.247197896242142
610 0.258350133895874
609 0.256949186325073
608 0.263433933258057
607 0.292127043008804
606 0.274327307939529
605 0.274680554866791
604 0.276172906160355
603 0.27874031662941
602 0.286770522594452
601 0.279874116182327
600 0.272173881530762
599 0.285809874534607
598 0.258576095104218
597 0.269306719303131
596 0.255612879991531
595 0.26107120513916
594 0.26353120803833
593 0.268686175346375
592 0.272857666015625
591 0.267679184675217
590 0.253770887851715
589 0.26812219619751
588 0.254640012979507
587 0.247395157814026
586 0.268924057483673
585 0.267214983701706
584 0.254888147115707
583 0.256547719240189
582 0.21364688873291
581 0.217437207698822
580 0.186386823654175
579 0.162579387426376
578 0.182082444429398
577 0.164271324872971
576 0.163796633481979
575 0.196603953838348
574 0.133258521556854
573 0.143430471420288
572 0.107962369918823
571 0.102929927408695
570 0.11338697373867
569 0.0845307558774948
568 0.0791487842798233
567 0.089537650346756
566 0.0560025423765182
565 0.0846716463565826
564 0.0631259828805923
563 0.0488521903753281
562 0.0606601759791374
561 0.050443708896637
560 0.0736347138881683
559 0.0783303081989288
558 0.0236960798501968
557 0.0626104474067688
556 0.0655613616108894
555 0.036089014261961
554 0.0916715115308762
553 0.106347687542439
552 0.0560448840260506
551 0.0373649820685387
550 0.0308923833072186
549 0.0214083585888147
548 0.0522543340921402
547 0.00257747620344162
546 0.0405677556991577
545 0.0116312671452761
544 0.0185370966792107
543 0.0389628522098064
542 0.0317402109503746
541 0.0745802372694016
540 0.0165568105876446
539 0
538 0.0588065013289452
537 0
536 0.00884053856134415
535 0.0464184805750847
534 0
533 0
532 0.0328307077288628
531 0
530 0.0675188526511192
529 0.0226764958351851
528 0.0373970493674278
527 0.0896106064319611
526 0.0782916322350502
525 0.132729828357697
524 0.21393695473671
523 0.2289077937603
522 0.270519435405731
521 0.349961191415787
520 0.426957815885544
519 0.497172981500626
518 0.522964179515839
517 0.560960531234741
516 0.609448671340942
515 0.586633920669556
514 0.617917478084564
513 0.573833346366882
512 0.535570979118347
511 0.510033011436462
510 0.418177366256714
509 0.423654973506927
508 0.355105429887772
507 0.321265608072281
506 0.342169493436813
505 0.292368829250336
504 0.269312083721161
503 0.298633396625519
502 0.2596455514431
501 0.276570707559586
500 0.278971910476685
499 0.229107171297073
498 0.263188093900681
497 0.250597417354584
496 0.274230867624283
495 0.265758723020554
494 0.247719526290894
493 0.277906209230423
492 0.240201145410538
491 0.21170449256897
490 0.221382409334183
489 0.214327096939087
488 0.22081270813942
487 0.208959966897964
486 0.138856738805771
485 0.177132606506348
484 0.157613784074783
483 0.116049207746983
482 0.145953476428986
481 0.128883004188538
480 0.110022611916065
479 0.101644910871983
478 0.0354784205555916
477 0.0853307321667671
476 0.0687622278928757
475 0.0489666536450386
474 0.0778625905513763
473 0.0565822087228298
472 0.0151421241462231
471 0.059931106865406
470 0.00698949210345745
469 0.051022969186306
468 0.00848548859357834
467 0
466 0.0267480872571468
465 0
464 0
463 0.0187575407326221
462 0
461 0
460 0
459 0
458 0
457 0
456 0
455 0
454 0
453 0
452 0
451 0
};
\addlegendentry{Spoiled}
\end{axis}

\end{tikzpicture}

